A Faster Exponential Time Algorithm for Bin Packing With a Constant Number of Bins via Additive Combinatorics

In the Bin Packing problem one is given $n$ items with weights $w_1,\ldots,w_n$ and $m$ bins with capacities $c_1,\ldots,c_m$. The goal is to find a partition of the items into sets $S_1,\ldots,S_m$ such that $w(S_j) \leq c_j$ for every bin $j$, where $w(X)$ denotes $\sum_{i \in X}w_i$. Bj\"orklund, Husfeldt and Koivisto (SICOMP 2009) presented an $\mathcal{O}^\star(2^n)$ time algorithm for Bin Packing. In this paper, we show that for every $m \in \mathbf{N}$ there exists a constant $\sigma_m >0$ such that an instance of Bin Packing with $m$ bins can be solved in $\mathcal{O}(2^{(1-\sigma_m)n})$ randomized time. Before our work, such improved algorithms were not known even for $m$ equals $4$. A key step in our approach is the following new result in Littlewood-Offord theory on the additive combinatorics of subset sums: For every $\delta >0$ there exists an $\varepsilon >0$ such that if $|\{ X\subseteq \{1,\ldots,n \} : w(X)=v \}| \geq 2^{(1-\varepsilon)n}$ for some $v$ then $|\{ w(X): X \subseteq \{1,\ldots,n\} \}|\leq 2^{\delta n}$.

==> Makefile <==
SOURCES := $(shell find $(SOURCEDIR) -name '*.tex')

all: main.pdf

main.pdf: $(SOURCES) main.bbl 
	pdflatex main.tex
	pdflatex main.tex

main.aux: $(SOURCES)
	pdflatex main.tex

main.bbl: bib.bib main.aux
	bibtex main

clean:
	rm -f img/*.log img/*.aux 
	rm -f *~ *.log *.out *.aux *.blg *.bbl *.gz

distclean: clean
	rm -f main.pdf

tar: clean
	bash -c "cd ..; tar -czf ${BASE}.tar.gz ${BASE}/*; mv ${BASE}.tar.gz ${BASE}"

spell:
	@for i in `find . -name "*.tex"` ; do \
		echo "------------ $$i --------------" ; \
		aspell list --lang=en --mode=tex --dont-tex-check-comments --personal=./blue-slownik.txt < $$i | sort | uniq ; \
done

diff:
	mkdir /tmp/cut-and-count-diff/
	python3 ~/latex-flatten.py main.tex /tmp/cut-and-count-diff/test.tex
	python3 ~/latex-flatten.py /tmp/cut-and-count-diff/test.tex /tmp/cut-and-count-diff/test2.tex
	python3 ~/latex-flatten.py /tmp/cut-and-count-diff/test2.tex /tmp/cut-and-count-diff/d2.tex
	git checkout $(branch-id)
	python3 ~/latex-flatten.py main.tex /tmp/cut-and-count-diff/test.tex
	python3 ~/latex-flatten.py /tmp/cut-and-count-diff/test.tex /tmp/cut-and-count-diff/test2.tex
	python3 ~/latex-flatten.py /tmp/cut-and-count-diff/test2.tex /tmp/cut-and-count-diff/d1.tex
	latexdiff /tmp/cut-and-count-diff/d1.tex /tmp/cut-and-count-diff/d2.tex > /tmp/cut-and-count-diff/diff.tex
	pdflatex /tmp/cut-and-count-diff/diff.tex
	git checkout master


==> chapters/hardercases.tex <==







